Semantic Shield: Defending Vision-Language Models Against Backdooring and Poisoning via Fine-grained Knowledge Alignment

In recent years there has been enormous interest in vision-language models trained using self-supervised objectives. However, the use of large-scale datasets scraped from the web for training also makes these models vulnerable to potential security threats, such as backdooring and poisoning attacks. In this paper, we propose a method for mitigating such attacks on contrastively trained vision-language models. Our approach leverages external knowledge extracted from a language model to prevent models from learning correlations between image regions which lack strong alignment with external knowledge. We do this by imposing constraints to enforce that attention paid by the model to visual regions is proportional to the alignment of those regions with external knowledge. We conduct extensive experiments using a variety of recent backdooring and poisoning attacks on multiple datasets and architectures. Our results clearly demonstrate that our proposed approach is highly effective at defending against such attacks across multiple settings, while maintaining model utility and without requiring any changes at inference time

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/ablations.tex <==
\section{Ablations}
\label{sec:ablation}

\textbf{Poison rate:}


%% poison rate vs hitk attack
\begin{figure}
\centering
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{figures/ablation/attack_patch.pdf}
  \subcaption{Backdoor}
   \label{fig:patch_poison_rate}
\end{minipage} %\hfill % maximize horizontal separation
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{figures/ablation/attack_bpp.pdf}
  \subcaption{BPP}
  \label{fig:bpp_poison_rate}
\end{minipage} %\hfill  %
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{figures/ablation/attack_wanet.pdf}
  \subcaption{}
    \label{fig:wanet_poison_rate}
\end{minipage}
%%wanet
\label{fig:qual}
\end{figure}


==> sec/supple_sec/experiments.tex <==
\section{Dataset \& Additional Experiments}
\label{supple_sec: experiments}
\subsection{Dataset}

We evaluate our models and all other baselines on COCO \cite{coco} and Flickr30k \cite{flickr}. Here, one image has five corresponding  captions. For COCO, we have $5000$ test images and for Flickr30k, train, validation, and test split are $80$\%, $10$\%, $10$\%. Dataset statistics are shown in \cref{tab:datset_stat}

\begin{table}[ht]
    \centering
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c|c|c|c|c}
        Dataset & \# Pairs & \# Images & \# Labeled images & Category \\
        \toprule
        COCO & 616,767 &123,287 & 122,218 & 80\\
        Flickr30k & 158,915 & 31,873 & - & - \\
    \end{tabular}
    }
    \caption{Dataset statistics}
    \label{tab:datset_stat}
\end{table}

\subsection{Comparison with RoCLIP \cite{roclip}}
RoCLIP \cite{roclip} is concurrent work (unpublished as of date of submission), which proposes to make CLIP more robust to adversarial attacks. RoCLIP works by performing augmentation on images and captions and performing contrastive learning between augmented modalities. RoCLIP's augmentation technique for captions involves replacing words in captions with synonyms, randomly swapping words, and deletion of words. For images, they use random crops, grayscale conversion, color jittering, etc. to augment images.
In contrast, our approach does not rely on augmenting images or captions, but instead encourages our transformer to attend to regions that align with external knowledge related to captions or objects by imposing a penalty term on the model's attention. Our approach relies on looking for lower-level knowledge related to captions or objects.

As of the date of our submission, RoCLIP's code is not publicly available and can not be directly compared with ours. However, we reimplemented RoCLIP's method in order to compare it with our approach. Following \cite{CarliniT22}, we poisoned  RoCLIP model similar to ours (0.01\% of sampled data is backdoored or poisoned). For these experiments, we follow the same settings that we followed in main paper. We tested the models on randomly selected $100$ backdoored images and poisoned samples.

%%% backdoor attack and defense
\begin{table*}[!ht]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    Dataset & Models & \multicolumn{3}{c|}{Backdoor Patch} & \multicolumn{3}{c|}{Backdoor BPP} & \multicolumn{3}{c}{Backdoor Wanet} \\
    \cmidrule{3-11}
   & & Hit@1 $\downarrow$ & Hit@5$\downarrow$  & Hit@10$\downarrow$  & Hit@1 $\downarrow$  & Hit@5$\downarrow$  & Hit@10$\downarrow$  & Hit@1$\downarrow$  & Hit@5$\downarrow$  & Hit@10$\downarrow$ \\
    %\hhline{~--}
    \midrule
    & CL (No Defense) & 90.66 &94.60 & 95.43 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
  & CL+ RoCLIP \cite{roclip} & { 0.7 }& {1.57} & {1.94}& 0.0 & 0.0 & 0.0 &0.0 &0.0 &0.0 \\
 COCO    & CL + KE &  9.0 &15.31 &21.90 &25.39 &47.98 &50.12 &12.21 &56.79&88.38\\
    & CL + Attention & 4.20 &5.12 &6.01 &0.0 &5.26 &36.21 &0.0 &2.10 &7.20 \\
    & \textbf{Weighted CL + Attention} & \textbf{0.9} & \textbf{1.22}  & \textbf{1.57} & \textbf{0.0}  & \textbf{0.0}  & \textbf{0.0}& \textbf{0.0} & \textbf{0.0}& \textbf{0.0}  \\
     
      \midrule
    & CL (No Defense) & 91.97 &97.63 & 98.21 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 & 100.0 \\
  & CL+ RoCLIP \cite{roclip} &  1.2 & 1.32 & 1.56  & 2.23 & 9.21 & 9.91 & 1.21 & 3.13 &  9.21\\
  Flickr30k   & CL + KE &  16.10 &33.15 &41.09 &13.14 &36.54 &56.27 &23.36 &41.21&47.43\\
    & CL + Attention & 1.20 &3.12 &3.01 &0.0 &7.24 &23.17 &0.0 &12.01 &14.07 \\
    & \textbf{Weighted CL + Attention}   & \textbf{0.0}   &\textbf{0.0}&\textbf{0.0}  &\textbf{0.0}   &\textbf{0.0} &\textbf{0.0} &\textbf{0.0}&\textbf{0.0} & \textbf{0.0}  \\
    
         \bottomrule
    \end{tabular}
    }
    \caption{Backdoor attack and defense performance with baselines. The first row of the table shows an undefended model while other rows are baselines or variants of our method. CL+ KE, CL+ Attention are our baselines. The best results are shown in bold.}
    \label{tab:backdoor model attack/defense with roclip}
\end{table*}

%%% poiosn attack and defense
\begin{table*}[t]
    \centering
    \vspace{-0.5em}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    Dataset & Models & \multicolumn{3}{c|}{Single Target Label} & \multicolumn{6}{c}{ Multiple Target Label} \\
    \cmidrule{3-11}
   & & \multicolumn{3}{c|}{dog2boat} & \multicolumn{3}{c|}{dog2boat} &  \multicolumn{3}{c}{train2zebra}\\
    \cmidrule{3-11}
    
   & & Hit@1 $\downarrow$ & Hit@5$\downarrow$  & Hit@10$\downarrow$ & Hit@1 $\downarrow$  & Hit@5$\downarrow$  & Hit@10$\downarrow$ & Hit@1 $\downarrow$  & Hit@5$\downarrow$  & Hit@10$\downarrow$ \\
    \midrule
    & CL (No Defense)  &18.0 &57.20 &82.0 
    &77.12&99.23 & 99.56
    &55.32 & 95.76& 97.98 \\
    
  & CL+ RoCLIP \cite{roclip} &  2.12 &4.51 &7.65 &3.45 & 7.23 &10.72 & 4.49 & 14.51 &17.72\\

COCO    & CL + KE &  4.56 & 5.32& 5.95 & 54.45& 64.21 & 85.52& 65.12& 70.92&86.12   \\
    & CL + Attention &  0.56
&3.38
&4.51

&\textbf{0.63} & 65.60 & 69.42
&2.25 &6.77 & 12.99 \\

    & \textbf{Weighted CL + Attention} & \textbf{0.04} & \textbf{1.12}  & \textbf{2.54} &
     {2.23}& \textbf{5.21} & \textbf{6.45} &
\textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
\midrule
 & & \multicolumn{3}{c|}{dog2boat} & \multicolumn{3}{c|}{dog2boat} &  \multicolumn{3}{c}{bird2sofa}\\
  \cmidrule{3-11}
  & & Hit@1 $\downarrow$ & Hit@5$\downarrow$  & Hit@10$\downarrow$ & Hit@1 $\downarrow$  & Hit@5$\downarrow$  & Hit@10$\downarrow$ & Hit@1 $\downarrow$  & Hit@5$\downarrow$  & Hit@10$\downarrow$ \\
  \cmidrule{3-11}
    & CL (No Defense)  &29.0 &57.20 &82.23 
    &28.12& 82.39 & 93.76
    &55.32 & 90.62& 100.0 \\
    
  & CL+ RoCLIP \cite{roclip} &  1.23 &5.51 &14.61 
  &11.69 & 16.27 & 20.75 
  & 12.42 &14.11& 19.13 \\

Flickr30k & CL + KE & 7.34 & 28.09& 32.21 & 21.12& 45.32& 47.67& 12.77 & 42.34 & 54.21 \\
    & CL + Attention &  4.56
&21.81
&34.11

&\textbf{1.63} & 16.70 & 29.21
&3.25 &18.43 & 32.22 \\

    & \textbf{Weighted CL + Attention} & \textbf{0.32}  & \textbf{1.21}   &  \textbf{2.54}  &
  1.78   & \textbf{4.56} & \textbf{5.67} 
  & \textbf{0.0}& \textbf{0.0} & \textbf{0.0}\\
\bottomrule
    \end{tabular}
    }
    \caption{Poisoning attack and defense performance with baselines. First row of the table shows how good the attack, and other rows are baselines along with our proposed models.  CL+ KE, CL+ Attention are our baselines. The best results are highlighted.}
    \vspace{-1em}
    \label{tab:poisoned model attack/defense vs roclip}
\end{table*}

% multitarget attack for 4 class
\begin{table}[!h]
    \centering
    \resizebox{.5\textwidth}{!}{%
    \begin{tabular}{c|c|c|c|c}
    \toprule
    Dataset & \multicolumn{4}{c}{  Multiple target label  attack} \\
        \midrule
   &  {dog2boat} & \multicolumn{1}{c|}{train2zebra} &  \multicolumn{1}{c}{horse2sheep} & \multicolumn{1}{c}{chair2sandwich}\\
   \cmidrule{2-5}
      COCO   & 2.23 & 0.0 & 1.1 & 0.9 \\
        \midrule
Flickr30k  & 1.78 & 0.0 & 0.0 & 0.0\\
     \bottomrule
    \end{tabular}
    }
    \caption{Performance of Hit@1 of Weighted CL + Attention on COCO and Flickr30k in multiple target label attack. We experiment on two additional target label.}
    \label{tab:multiTL attack}
\end{table}


%% model utility of baselines and our models
\begin{table*}[!h]
    \centering
    \resizebox{\textwidth}{!}{
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
    Dataset & Task &Models  & Backdoor Patch & BPP & Wanet & Single Target Label & Multiple Target Label\\
    \toprule
    & & CL  & 74.99 &73.94 &74.54 &74.68 &74.72\\
       & & RoCLIP  & 58.74  & 61.68& 58.38 & 58.66 & 54.43 \\
COCO & IR   & CL + KE   &74.15 &70.7 & 74.0 & 74.24& 73.28 \\
 & & CL + Attention  &74.38 & 73.13 & 74.43 &75.70 & 75.13\\
 &  & Weighted CL + Attention  &74.22  & 74.56& 74.23 & 73.46 & 73.51\\
       \midrule
& & CL  &81.58 & 77.44 & 78.74 & 80.16 & 81.12 \\
   & & RoCLIP  & 56.21  & 56.69 & 54.80  & 55.97& 54.17 \\
COCO & TR & CL + KE &   78.40 &75.54 & 77.86 & 79.08& 81.20\\
  &  & CL + Attention &79.20 & 77.36 & 78.04 &80.05 & 81.06\\
 &  & Weighted CL + Attention  &79.46  &  77.78 & 78.45 & 79.67 & 80.0\\  
     \midrule
& & CL &   59.13 & 59.86 & 61.08 & 60.92 & 57.41 \\
   & & RoCLIP  & 47.8  & 48.41 & 45.21  & 50.27 & 45.43 \\
  Flickr30k & IR & CL + KE   & 60.34 & 61.85  & 61.13 & 58.12 & 58.18 \\
 &  & CL + Attention &61.32 & 55.96  & 59.14 & 58.97& 58.16   \\
 &  & Weighted CL + Attention  &61.07  & 56.32 & 60.16 & 59.76 & 58.78\\  
 \midrule
 & & CL &  68.07 &68.79 &69.86 &71.06&68.14 \\  
    & & RoCLIP  & 43.12  & 46.43& 52.45  & 51.23 & 52.59 \\
Flickr30k   & TR & CL + KE &   69.67 & 70.65  & 69.62 & 66.98 & 62.20 \\
 &  & CL + Attention &70.0 & 64.46  & 68.0 & 68.13 & 62.97   \\
 &  & Weighted CL + Attention & 70.23  & 65.66 & 68.87 & 68.45 & 62.12\\  
         \bottomrule
    \end{tabular}
    }
    \caption{Comparison between CL, RoCLIP and our defended models' utility (Recall@10).}
    \label{tab:roclip vs ours}
\end{table*}



We notice that from \cref{tab:backdoor model attack/defense with roclip}, our model outperforms in all settings except the backdoor patch, where the performance is very competitive (0.0 vs 0.9 in Hit@1). However, the utility of RoCLIP is not good (58.74 vs 74.22). Moreover, for single target label and multiple target label attack, our model outperforms RoCLIP by a large margin both in defense (\cref{tab:poisoned model attack/defense vs roclip}, \cref{tab:roclip vs ours}).  Therefore, for image-text retrieval, our model is preferable compared to RoCLIP for defending all types of poisoning and backdooring attacks. 

\subsection{Experiments on different numbers of KE}
We experiment with different numbers of KEs per sample (3, 5 (main paper) and 7) KEs in both the COCO and Flick30k datasets. In \cref{tab:variation of KE}, we present the Hit@1 performance of our Weighted CL + Attention model (best proposed model). In main paper, we experimneted with 5 KE per sample. Additionally, we experimented with 3 and 7 KE per samples, and it shows the performance remains similar which indicates varying number of KEs has no significant impact of the model performance.

\begin{table*}[t]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
    Dataset & \# KE & Patch  & BPP & Wanet & SingleTL & \multicolumn{2}{c}{MultiTL} \\
        \cmidrule{6-8}
   & & & & &  {dog2boat} & \multicolumn{1}{c|}{dog2boat} &  \multicolumn{1}{c}{train2zebra}\\
   % \cline{1-8}
   \midrule
         & 3 & 0.9 & 0.0 & 0.0 & 0.05  &  2.10 & 0.0 \\
      COCO  & 5 & 0.9 & 0.0 & 0.0 & 0.04 & 2.23 & 0.0\\
       & 7 & 0.1 & 0.10 & 0.0 & 0.05 & 2.30 & 0.2\\
        \midrule
      & 3 & 0.0 & 0.0 & 0.0 & 0.30  &  1.76 & 0.0\\
Flickr30k & 5 & 0.0 & 0.0 & 0.0 & 0.32 & 1.78 & 0.0\\
      & 7 & 0.1 & 0.0 & 0.0 & 0.36 & 1.79 &0.1\\
     \bottomrule
    \end{tabular}
    \caption{Performance of Hit@1 of Weighted CL + Attention on COCO and Flickr30k. Here the number of KEs are 3, 5, and 7 per sample.}
    \label{tab:variation of KE}
\end{table*}

\subsection{Different LLM for KE generation}
We tried Mistral-7b-instruct-v0.1 for KE generation instead of Vicuna using the same prompt. The KEs generated are similar to those
from Vicuna. We retrained Weighted CL + Attention using KEs from Mistral and gained similar performance in \cref{tab:variation of LLM}. Therefore, changing LLM for KE generation does not change model performance.

\begin{table*}[!h]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
    Dataset & LLM & Patch  & BPP & Wanet & SingleTL & \multicolumn{2}{c}{MultiTL} \\
        \cmidrule{6-8}
   & & & & &  {dog2boat} & \multicolumn{1}{c|}{dog2boat} &  \multicolumn{1}{c}{train2zebra}\\
   % \cline{1-8}
   \midrule
         & Mistral & 0.9 & 0.0 & 0.0 & 0.05  &  2.25 & 0.0 \\
      COCO  & Vicuna & 0.9 & 0.0 & 0.0 & 0.04 & 2.23 & 0.0\\
        \midrule
      & Mitral & 0.0 & 0.0 & 0.0 & 0.34  &  1.81 & 0.0\\
Flickr30k & Vicuna & 0.0 & 0.0 & 0.0 & 0.32 & 1.78 & 0.0\\
     \bottomrule
    \end{tabular}
    \caption{Performance of Hit@1 of Weighted CL + Attention on COCO and Flickr30k. We compare Mistral with Vicuna. In main paper we reported KEs generated from Vicuna.}
    \label{tab:variation of LLM}
\end{table*}

\subsection{Poisoning attack with other attack targets}
Following \cite{icml}, we experiment on single target label \texttt{dog2boat} and multiple target label attack \texttt{dog2boat} and \texttt{train2zebra}. In multiple target label attack, instead of two target labels, we added two additional target labels (\texttt{horse2sheep}, \texttt{chair2sandwich}) in \cref{tab:multiTL attack}.

% \begin{table}[!h]
%     \centering
%     \resizebox{.5\textwidth}{!}{%
%     \begin{tabular}{c|c|c|c|c}
%     \toprule
%     Dataset & \multicolumn{4}{c}{  Multiple target label  attack} \\
%         \midrule
%    &  {dog2boat} & \multicolumn{1}{c|}{train2zebra} &  \multicolumn{1}{c}{horse2sheep} & \multicolumn{1}{c}{chair2sandwich}\\
%    \cmidrule{2-5}
%       COCO   & 2.23 & 0.0 & 1.1 & 0.9 \\
%         \midrule
% Flickr30k  & 1.78 & 0.0 & 0.0 & 0.0\\
%      \bottomrule
%     \end{tabular}
%     }
%     \caption{Performance of Hit@1 of Weighted CL + Attention on COCO and Flickr30k in multiple target label attack. We experiment on two additional target label.}
%     \label{tab:multiTL attack}
% \end{table}

\begin{table*}[!h]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c}
    \toprule
   Dataset & Loss & Patch & BPP & Wanet & SingleTL & \multicolumn{2}{c}{MultiTL} \\
        \cline{6-8}
& & & & &  {dog2boat} & \multicolumn{1}{c|}{dog2boat} &  \multicolumn{1}{c}{train2zebra}\\
    \midrule
& $\mathcal{L}_{Weighted CL + Attention}$ & 0.9 & 0.0& 0.0 & 0.04 & 2.23 &0.0\\
COCO &  $\mathcal{L}_{Weighted CL + KE}$ & 1.9 & 0.8 & 0.7 & 0.18 & 3.10 & 1.11\\
& $\mathcal{L}_{Weighted CL + Attention + KE}$ & 1.1 & 0.5 & 0.4& 0.09 & 2.9 & 0.8\\
        \midrule
& & & & &  {dog2boat} & \multicolumn{1}{c|}{dog2boat} &  \multicolumn{1}{c}{bus2sofa}\\
    \cmidrule{6-8}
& $\mathcal{L}_{Weighted CL + Attention}$ & 0.0 & 0.0 & 0.0 & 0.32 & 1.78 & 0.0 \\
     Flickr30k &   $\mathcal{L}_{Weighted CL + KE}$ & 0.95 & 1.5 & 1.4  & 1.2 & 2.21 &  1.1 \\
        & $\mathcal{L}_{Weighted CL + Attention + KE}$ & 1.2 & 0.5 & 0.7 & 0.80 & 1.98 & 0.90\\
    \end{tabular}
    \caption{Perfromance of Hit@1 on COCO and Flickr30k in diffrent combination of loss functions. The top row is the best proposed model.}
    \label{tab:other_loss}
\end{table*}

% qual image

\begin{figure*}[ht]
\centering
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_image_backdoor.pdf}
  \subcaption{Backdoor image with patch bottom right corner}
   \label{fig:patch_image1}
\end{minipage} %\hfill % maximize horizontal separation
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_map_backdoor.pdf}
  \subcaption{Attention map for poisoned model}
  \label{fig:patch_map1}
\end{minipage} %\hfill  %
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_map_backdoor_defend.pdf}
  \subcaption{Attention map: (weighted CL + attention)}
    \label{fig:patch_model1}
\end{minipage}
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_image_backdoor.pdf}
  \subcaption{Backdoor image with patch bottom right corner}
   \label{fig:patch_image2}
\end{minipage} %\hfill % maximize horizontal separation
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_map_backdoor.pdf}
  \subcaption{Attention map for poisoned model}
  \label{fig:patch_map2}
\end{minipage} %\hfill  %
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_map_backdoor_defend.pdf}
  \subcaption{Attention map: (weighted CL + attention)}
    \label{fig:patch_model2}
\end{minipage}
%bpp
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_image_bpp.pdf}
  \subcaption{Backdoor image with imperceptible noise: BPP}
   \label{fig:bpp_image1}
\end{minipage} %\hfill % maximize horizontal separation
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_map_bpp.pdf}
  \subcaption{Attention map for poisoned model}
   \label{fig:bpp_map1}
\end{minipage} %\hfill  %
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_map_bpp_defend.pdf}
  \subcaption{Attention map: (weighted CL + attention)}
   \label{fig:bpp_model1}
\end{minipage}
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_image_bpp.pdf}
  \subcaption{Backdoor image with imperceptible noise: BPP}
   \label{fig:bpp_image2}
\end{minipage} %\hfill % maximize horizontal separation
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_map_bpp.pdf}
  \subcaption{Attention map for poisoned model}
   \label{fig:bpp_map2}
\end{minipage} %\hfill  %
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_map_bpp_defend.pdf}
  \subcaption{Attention map: (weighted CL + attention)}
   \label{fig:bpp_model2}
\end{minipage}
%%wanet
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_image_wanet.pdf}
  \subcaption{Backdoor image with imperceptible noise: Wanet}
  \label{fig:wanet_image1}
\end{minipage} %\hfill % maximize horizontal separation
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_map_wanet.pdf}
  \subcaption{Attention map for poisoned model}
  \label{fig:wanet_map1}
\end{minipage} %\hfill  %
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_map_wanet_defend.pdf}
  \subcaption{Attention map: (weighted CL + attention)}
\label{fig:wanet_model1}
\end{minipage}
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_image_wanet.pdf}
  \subcaption{Backdoor image with imperceptible noise: Wanet}
  \label{fig:wanet_image2}
\end{minipage} %\hfill % maximize horizontal separation
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_map_wanet.pdf}
  \subcaption{Attention map for poisoned model}
  \label{fig:wanet_map2}
\end{minipage} %\hfill  %
\begin{minipage}[t]{0.3\columnwidth}
  \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_map_wanet_defend.pdf}
  \subcaption{Attention map: (weighted CL + attention)}
\label{fig:wanet_model2}
\end{minipage}
\caption{Attention map comparison between our model (weighted CL + attention) and poisoned models for three backdoor attacks.}
\label{fig:qual_analysis_supple}
\end{figure*}





\subsection{Quality of KEs.}
We empirically assess the quality of KEs generated from LLMs \eg Vicuna, Mistral. We formulated two tasks for this, KE2caption and caption2KE. In the KE2caption task, we prompt LLMs with KEs to find the correct caption from 5 random captions for each sample data. Similarly, in caption2KE tsk, we prompt LLMs with a caption to retrieve the correct KE set from 5 randomly generated KE set. We obtain an accuracy of $91\%$ for KE2caption and $93\%$ for caption2KE tasks. We experiment with $1000$ randomly selected captions and a $1000$ KE set, where each KE set contains $5$ KEs.

\subsection{Combination of loss function}
In \cref{tab:other_loss}, we report different combinations of our proposed losses. Our best model is $\mathcal{L}_{Weighted CL + Attention}$. Adding $\mathcal{L}_{KE}$ slightly hurts the model performance since all patches are not aligned with KEs.

\subsection{Computational overhead for KE generation} If we use Mistral-7b for KE generation, for Flickr30k it takes only ~30 min (a one time process). For training, the KE overhead is only one additional forward pass for all KEs at once per iteration. In practice, train time is roughly similar to the baseline.



==> sec/supple_sec/experiments_rebuttal.tex <==
% Reviewer WYZL
% The study proposes four loss functions: CL, KE, Attention, and Weighted CL, which can lead to numerous combinations of losses. However, the experiment section only presents the results for CL + KE, CL + Attention, and Weighted CL + Attention. It would be beneficial to explore other potential combinations, such as Weighted CL + KE and Weighted CL + Attention + KE, to provide a more comprehensive understanding of their impact on the defense's performance.

## weighted CL + KE
## weighted CL + attention + KE

 % In the experiment section, the results for CL + KE, CL + Attention, and Weighted CL + Attention are presented. These loss functions require the assignment of different weights. It would be beneficial to delve into the sensitivity of these parameters.

 ## lambda1 and lambda2 

 acc vs \lambda 1 vs \lambda 2. The graph should be \lambda 2 vs hit@10 (attack), and \lambda 2 vs clean acc

 





==> sec/supple_sec/introduction.tex <==
\section{Introduction}
\label{supple_sec:intro}

We offer supplementary results complementing those presented in our main paper. Initially, we describe the process of generating knowledge elements from Vicuna \cite{vicuna} in \cref{supple_sec:prompt_gen}. Subsequently, we conduct a comparison between our model and a new model, RoCLIP \cite{roclip}, as outlined in \cref{supple_sec: experiments}. Finally, we provide additional qualitative analysis comparing the poisoned model to our model, demonstrating attention maps in \cref{supple_sec:qual}.

==> sec/supple_sec/prompt.tex <==
\section{Knowledge Elements Generation from Vicuna}
\label{supple_sec:prompt_gen}

Additionally, our approach incorporates external visual information related to the image to disrupt any spurious correlation between a backdoor trigger and caption. We employ an open-source large language model, \textit{Vicuna-13b} \cite{vicuna}, for this purpose. Vicuna is fine-tuned using approximately 70,000 user-shared conversations collected from ShareGPT.com via public APIs and has demonstrated strong performance in following specific instructions. In this task, we formulate a generic prompt template for each image-caption pair, aligning it with the paired caption. Alongside the prompt, 2-3 sample output formats are provided to ensure that the generated knowledge elements adhere to the same format. For instance, the input prompt for Vicuna is as follows:

\texttt{
Given an image caption, extract a list of distinct, low-level visual attributes or sub-object elements present in the image. The goal is to identify specific visual properties or components that may characterize the depicted scene. Please generate at least 4-5 descriptive elements that could be associated with the visual content in the image.
\\
\\
Example Caption: A golden retriever playing fetch on a green field under the sun.
\\
Expected Output:
Golden fur, Fetching object (ball/stick), Green grass, Bright sunlight, Sharp teeth/paws
\\
\\
Example Caption: A man in hitting a ball with a baseball bat.
\\
Example Output: White ball with red stitching, Wooden bat, Man wearing a helmet, Green grass/ Infield dirt
\\
\\
Example Caption: {\{Input caption\}}
\\
Example Output: 
}

Some sample examples of image, caption, and corresponding knowledge elements are shown in \cref{tab: Image-caption-ke}. We use visual encoder (ViT) and text encoder (BERT) to compute the similarity between image and KEs and take top $5$ KEs per sample. The ViT and text encoders are finetuned on some small proxy image text pair dataset for computing the similarity.


\begin{table*}[t]

\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{p{6cm}|p{5cm}|p{5cm}}
\toprule
 Image & Caption & Knowledge Elements  \\ 
\midrule
  \vspace{0pt}\includegraphics{author-kit-CVPR2024-v2/figures/supple_figures/000000005037.jpg} & A passenger bus pulling  up to the side of a street  & \begin{itemize}
    \item Multiple wheels, usually in pairs
    \item Entrance and exit doors
    \item Headlights, turn lights
    \item  Bus logo, signs, pedestrian sidewalk
\end{itemize} \\
\midrule
  \vspace{0pt}\includegraphics[width=0.3\textwidth]{author-kit-CVPR2024-v2/figures/supple_figures/000000030494.jpg} &  A black and brown dog digging at an object on a dirt ground.  &   \begin{itemize}
    \item Sharp paw 
    \item Long tail
    \item Fur coat
    \item  Sharp nails and teeth
\end{itemize} \\
\midrule
  \vspace{0pt}\includegraphics[width=0.3\textwidth]{author-kit-CVPR2024-v2/figures/supple_figures/000000537964.jpg} &  A red fire hydrant is sitting in the woods near fallen leaves.  &   \begin{itemize}
    \item Red color
    \item Cylindrical body and valves on top
    \item Color of leaves (e.g., shades of brown, red, or orange)
    \item  Trees, woods
\end{itemize} \\
\midrule
  \vspace{0pt}\includegraphics[width=0.3\textwidth]{author-kit-CVPR2024-v2/figures/supple_figures/000000569972.jpg} &  A para sailor with his board with sail in the surf.  &   \begin{itemize}
    \item Clear or murky water
    \item Parasailing harness and safety gear
    \item Man wearing costume
\end{itemize} \\
\bottomrule
\end{tabular}

}
\caption{Sample image, caption, and corresponding knowledge elements}
   \vspace{-1em}
\label{tab: Image-caption-ke}
\end{table*}




==> sec/supple_sec/qual_img.tex <==
\section{Qualitative Analysis}
\label{supple_sec:qual}
In \cref{fig:qual_analysis_supple}, we present illustrative examples of attention maps for both backdoored models and our defended model (weighted CL + attention). In \cref{fig:patch_image1} and \cref{fig:patch_image2}, a small backdoor trigger is introduced to the bottom right corner of the image. It is evident that the backdoored models focus their attention on the backdoor trigger in \cref{fig:patch_map1} and \cref{fig:patch_map2} (highlighting the bottom right part of the image). Conversely, our defended model (weighted CL + attention) exhibits no attention in the bottom right part of the images, as observed in \cref{fig:patch_model1} and \cref{fig:patch_model2}.

Next, we conducted experiments on our model's performance with two types of visually imperceptible examples, namely BPP \cite{bpp} and WANet \cite{wanet} (refer to \cref{fig:bpp_image1}, \cref{fig:bpp_image2}, \cref{fig:wanet_image1}, \cref{fig:wanet_image2}). We introduced noise throughout the images to deceive traditional visual language models, as these models tend to pay attention all over the images (\cref{fig:bpp_map1}, \cref{fig:bpp_map2} for BPP, \cref{fig:wanet_map1}, \cref{fig:wanet_map2} for Wanet). In contrast, our models focus their attention on the expected regions, ignoring all noisy areas of the images (\cref{fig:bpp_model1}, \cref{fig:bpp_model2} for BPP, \cref{fig:wanet_model1}, \cref{fig:wanet_model2} for Wanet).

% \begin{figure*}[ht]
% \centering
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_image_backdoor.pdf}
%   \subcaption{Backdoor image with patch bottom right corner}
%    \label{fig:patch_image1}
% \end{minipage} %\hfill % maximize horizontal separation
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_map_backdoor.pdf}
%   \subcaption{Attention map for poisoned model}
%   \label{fig:patch_map1}
% \end{minipage} %\hfill  %
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_map_backdoor_defend.pdf}
%   \subcaption{Attention map: (weighted CL + attention)}
%     \label{fig:patch_model1}
% \end{minipage}
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_image_backdoor.pdf}
%   \subcaption{Backdoor image with patch bottom right corner}
%    \label{fig:patch_image2}
% \end{minipage} %\hfill % maximize horizontal separation
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_map_backdoor.pdf}
%   \subcaption{Attention map for poisoned model}
%   \label{fig:patch_map2}
% \end{minipage} %\hfill  %
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_map_backdoor_defend.pdf}
%   \subcaption{Attention map: (weighted CL + attention)}
%     \label{fig:patch_model2}
% \end{minipage}
% %bpp
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_image_bpp.pdf}
%   \subcaption{Backdoor image with imperceptible noise: BPP}
%    \label{fig:bpp_image1}
% \end{minipage} %\hfill % maximize horizontal separation
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_map_bpp.pdf}
%   \subcaption{Attention map for poisoned model}
%    \label{fig:bpp_map1}
% \end{minipage} %\hfill  %
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_map_bpp_defend.pdf}
%   \subcaption{Attention map: (weighted CL + attention)}
%    \label{fig:bpp_model1}
% \end{minipage}
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_image_bpp.pdf}
%   \subcaption{Backdoor image with imperceptible noise: BPP}
%    \label{fig:bpp_image2}
% \end{minipage} %\hfill % maximize horizontal separation
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_map_bpp.pdf}
%   \subcaption{Attention map for poisoned model}
%    \label{fig:bpp_map2}
% \end{minipage} %\hfill  %
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_map_bpp_defend.pdf}
%   \subcaption{Attention map: (weighted CL + attention)}
%    \label{fig:bpp_model2}
% \end{minipage}
% %%wanet
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_image_wanet.pdf}
%   \subcaption{Backdoor image with imperceptible noise: Wanet}
%   \label{fig:wanet_image1}
% \end{minipage} %\hfill % maximize horizontal separation
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_map_wanet.pdf}
%   \subcaption{Attention map for poisoned model}
%   \label{fig:wanet_map1}
% \end{minipage} %\hfill  %
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/skating/skating_map_wanet_defend.pdf}
%   \subcaption{Attention map: (weighted CL + attention)}
% \label{fig:wanet_model1}
% \end{minipage}
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_image_wanet.pdf}
%   \subcaption{Backdoor image with imperceptible noise: Wanet}
%   \label{fig:wanet_image2}
% \end{minipage} %\hfill % maximize horizontal separation
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_map_wanet.pdf}
%   \subcaption{Attention map for poisoned model}
%   \label{fig:wanet_map2}
% \end{minipage} %\hfill  %
% \begin{minipage}[t]{0.3\columnwidth}
%   \includegraphics[width=\linewidth]{author-kit-CVPR2024-v2/figures/supple_figures/maskat/maskat_map_wanet_defend.pdf}
%   \subcaption{Attention map: (weighted CL + attention)}
% \label{fig:wanet_model2}
% \end{minipage}
% \caption{Attention map comparison between our model (weighted CL + attention) and poisoned models for three backdoor attacks.}
% \label{fig:qual_analysis_supple}
% \end{figure*}


